Flashlights: More than A Dozen High-Significance Microlensing Events of Extremely Magnified Stars in Galaxies at Redshifts z=0.7-1.5

Once only accessible in nearby galaxies, we can now study individual stars across much of the observable universe aided by galaxy-cluster gravitational lenses. When a star, compact object, or multiple such objects in the foreground galaxy-cluster lens become aligned, they can magnify a background individual star, and the timescale of a magnification peak can limit its size to tens of AU. The number and frequency of microlensing events therefore opens a window into the population of stars and compact objects, as well as high-redshift stars. To assemble the first statistical sample of stars in order to constrain the initial mass function (IMF) of massive stars at redshift z=0.7-1.5, the abundance of primordial black holes in galaxy-cluster dark matter, and the IMF of the stars making up the intracluster light, we are carrying out a 192-orbit program with the Hubble Space Telescope called "Flashlights," which is now two-thirds complete owing to scheduling challenges. We use the ultrawide F200LP and F350LP long-pass WFC3 UVIS filters and conduct two 16-orbit visits separated by one year. Having an identical roll angle during both visits, while difficult to schedule, yields extremely clean subtraction. Here we report the discovery of more than a dozen bright microlensing events, including multiple examples in the famous "Dragon Arc" discovered in the 1980s, as well as the "Spocks" and "Warhol" arcs that have hosted already known supergiants. The ultradeep observer-frame ultraviolet-through-optical imaging is sensitive to hot stars, which will complement deep James Webb Space Telescope infrared imaging. We are also acquiring Large Binocular Telescope LUCI and Keck-I MOSFIRE near-infrared spectra of the highly magnified arcs to constrain their recent star-formation histories.

==> Flashlights Initial Results(1)/institutions.tex <==
\newcommand{\Chiba}{Center for Frontier Science, Chiba University, 1-33 Yayoi-cho, Inage-ku, Chiba 263-8522, Japan}
\newcommand{\ChibaPhys}{Department of Physics, Graduate School of Science, Chiba University, 1-33 Yayoi-Cho, Inage-Ku, Chiba 263-8522, Japan}
\newcommand{\EarlyUniverse}{Research Center for the Early Universe, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\HongKong}{Department of Physics, The University of Hong Kong, Pokfulam Road, Hong Kong}
\newcommand{\ENS}{Laboratoire de Physique de l’Ecole Normale Supérieure, ENS, Université PSL, CNRS, Sorbonne Université, Université de Paris, Paris, France}
\newcommand{\HubbleFellow}{Hubble Fellow}
\newcommand{\Packard}{Packard Fellow}
\newcommand{\CalTech}{California Institute of Technology, 1200 East California Boulevard, Pasadena, CA 91125, USA}
\newcommand{\IFCA}{\Cantabria}
\newcommand{\UBasque}{Department of Theoretical Physics, University of the Basque Country, Bilbao 48080, Spain}
\newcommand{\JHU}{Department of Physics and Astronomy, The Johns Hopkins University, 3400 N. Charles St., Baltimore, MD 21218, USA}
\newcommand{\Michigan}{Department of Astronomy, University of Michigan, 1085 S. University Avenue, Ann Arbor, MI 48109, USA}
\newcommand{\UCDavis}{Department of Physics, University of California, Davis, 1 Shields Avenue, Davis, CA 95616, USA}
\newcommand{\UCLA}{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095}
\newcommand{\USC}{Department of Physics and Astronomy, University of South Carolina, 712 Main St., Columbia, SC 29208, USA}
\newcommand{\RCEU}{Research Center for the Early Universe, University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\newcommand{\TokyoPhys}{Department of Physics, University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\newcommand{\IPMU}{Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU, WPI), University of Tokyo, 5-1-5 Kashiwanoha, Kashiwa, Chiba 277-8583, Japan}
\newcommand{\TokyoAstro}{Department of Astronomy, Graduate School of Science, The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\newcommand{\EarlyTokyo}{Research Center for the Early Universe, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\DARK}{Dark Cosmology Centre, Niels Bohr Institute, University of Copenhagen, Juliane Maries Vej 30, DK-2100 Copenhagen, Denmark} 
\newcommand{\INFN}{INFN, Sezione di Bologna, Viale Berti Pichat 6/2, I-40127 Bologna, Italy}
\newcommand{\EHU}{Fisika Teorikoa, Zientzia eta Teknologia Fakultatea, Euskal Herriko Unibertsitatea UPV/EHU}
\newcommand{\Basque}{IKERBASQUE, Basque Foundation for Science, Alameda Urquijo, 36-5 48008 Bilbao, Spain}
\newcommand{\Berkeley}{Department of Astronomy, University of California, Berkeley, CA 94720-3411, USA}
\newcommand{\STScI}{Space Telescope Science Institute, 3700 San Martin Dr., Baltimore, MD 21218, USA}
\newcommand{\Milano}{Dipartimento di Fisica, Universit\'a degli Studi di Milano, via Celoria 16, I-20133 Milano, Italy}
\newcommand{\Ferrara}{Dipartimento di Fisica e Scienze della Terra, Universit\'a degli Studi di Ferrara, via Saragat 1, I-44122, Ferrara, Italy}
\newcommand{\INAF}{INAF, Osservatorio Astronomico di Trieste, via Bazzoni 2, 34124 Trieste, Italy}
\newcommand{\UCSB}{Department of Physics, University of California, Santa Barbara, CA 93106-9530, USA}
\newcommand{\SantaBarbara}{\UCSB}
\newcommand{\Kapteyn}{Kapteyn Astronomical Institute, University of Groningen, Postbus 800, 9700 AV Groningen, the Netherlands}
\newcommand{\IAP}{Institut Astrophysique de Paris, UMR7095 CNRS-Universit\'{e} Pierre et Marie Curie, 98bis bd Arago, F-75014 Paris, France}
\newcommand{\ASIAA}{Institute of Astronomy and Astrophysics, Academia Sinica, P.O. Box 23-141, Taipei 10617, Taiwan}
\newcommand{\TokyoKashiwa}{Institute for Cosmic Ray Research, The University of Tokyo, Kashiwa, Chiba 277-8582, Japan}
\newcommand{\Munich}{University Observatory Munich, Scheinerstrasse 1, D-81679 Munich, Germany} 
\newcommand{\KICPStanford}{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, 452 Lomita Mall, Stanford, CA 94305, USA}
\newcommand{\Andalucia}{Instituto de Astrof\'isica de Andaluc\'ia (CSIC), E-18080 Granada, Spain}
\newcommand{\SaoPaulo}{Instituto de Astronomia, Geof\'isica e Ci\^encias Atmosf\'ericas, Universidade de S\~ao Paulo, Cidade Universit\'aria, 05508-090, S\~ao Paulo, Brazil}
\newcommand{\AMNH}{Department of Astrophysics, American Museum of Natural History, Central Park West and 79th Street, New York, NY 10024, USA}
\newcommand{\NYU}{Center for Cosmology and Particle Physics, New York University, New York, NY 10003, USA}
\newcommand{\Arizona}{Department of Astronomy, University of Arizona, Tucson, AZ 85721, USA}
\newcommand{\Rutgers}{Department of Physics and Astronomy, Rutgers, The State University of New Jersey, Piscataway, NJ 08854, USA}
\newcommand{\NOAO}{National Optical Astronomical Observatory, Tucson, AZ 85719, USA}
\newcommand{\LCO}{Las Cumbres Observatory, 6740 Cortona Dr., Suite 102, Goleta, CA 93117, USA}
\newcommand{\IllinoisAstro}{ Astronomy Department, University of Illinois at Urbana-Champaign, 1002 W.\ Green Street, Urbana, IL 61801, USA }
\newcommand{\IllinoisPhysics}{ Department of Physics, University of Illinois at Urbana-Champaign, 1110 W.\ Green Street, Urbana, IL 61801, USA }
\newcommand{\UTAustin}{Department of Astronomy, University of Texas at Austin, Austin, TX 78712, USA}
\newcommand{\Stockholm}{The Oskar Klein Centre, Department of Astronomy, Stockholm University, AlbaNova, 10691, Stockholm, Sweden} 
\newcommand{\Cantabria}{IFCA, Instituto de F\'isica de Cantabria (UC-CSIC), Av. de Los Castros s/n, 39005 Santander, Spain}
\newcommand{\FisikaTeorika}{IFCA, Instituto de F\'isica de Cantabria (UC-CSIC), Av. de Los Castros s/n, 39005 Santander, Spain}
\newcommand{\IKERBASQUE}{Ikerbasque Foundation, University of the Basque Country, DIPC Donostia, Spain}
\newcommand{\IfA}{Institute for Astronomy, University of Hawaii, 2680 Woodlawn Drive, Honolulu, HI 96822-1839, USA}
\newcommand{\TohokuAstInst}{Astronomical Institute, Tohoku University, Aramaki, Aoba, Sendai 980-8578, Japan}
\newcommand{\TohokuAdvanced}{Institute for International Advanced Research and Education, Tohoku University, Aramaki, Aoba, Sendai 980-8578, Japan}
\newcommand{\UCM}{Departamento de Astrof\'isica, Facultad de CC. F\'isicas, Universidad Complutense de Madrid, E-28040 Madrid, Spain}
\newcommand{\UArizona}{Steward Observatory, University of Arizona, 933 N. Cherry Ave., Tucson, AZ 85721, USA}
\newcommand{\Goddard}{Astrophysics Science Division, NASA Goddard Space Flight Center, Mail Code 661, Greenbelt, MD 20771, USA}
\newcommand{\UMD}{Joint Space-Science Institute, University of Maryland, College Park, MD 20742, USA}
\newcommand{\UCSC}{Department of Astronomy and Astrophysics, UCO/Lick Observatory, University of California, 1156 High Street, Santa Cruz, CA 95064, USA}
\newcommand{\UWash}{Department of Astronomy, University of Washington, Box 351580, Seattle, WA, 98195, USA}
\newcommand{\Amsterdam}{Anton Pannekoek Institute for Astronomy, University of Amsterdam, NL-1090 GE Amsterdam, the Netherlands}
\newcommand{\IAGUSP}{Instituto de Astronomia, Geof\'isica e Ci\^encias Atmosf\'ericas, Universidade de S\~ao Paulo, 05508-090, S\~ao Paulo, Brazil}
\newcommand{\DurhamExtra}{Centre for Extragalactic Astronomy, Department of Physics, Durham University, Durham DH1 3LE, U.K.}
\newcommand{\DurhamCosmo}{Institute for Computational Cosmology, Durham University, South Road, Durham DH1 3LE, U.K.}
\newcommand{\Durban}{Astrophysics and Cosmology Research Unit, School of Mathematical Sciences, University of KwaZulu-Natal, Durban 4041, South Africa}
\newcommand{\EPFL}{Laboratoire d'Astrophysique, Ecole Polytechnique Federale de Lausanne (EPFL), Observatoire de Sauverny, CH-1290 Versoix, Switzerland}
\newcommand{\Oxford}{Department of Physics, University of Oxford, Keble Road, Oxford OX1 3RH, UK}
\newcommand{\JPL}{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA 91109, USA}
\newcommand{\Lyon}{Univ Lyon, Univ Lyon1, ENS de Lyon, CNRS, Centre de Recherche Astrophysique de Lyon UMR5574, F-69230, Saint-Genis-Laval, France}
\newcommand{\AIP}{Leibniz-Institut fur Astrophysik Potsdam (AIP), An der Sternwarte 16, 14482 Potsdam, Germany}
\newcommand{\UMich}{University of Michigan, Department of Astronomy, 1085 South University Avenue, Ann Arbor, MI 48109-1107, USA}
\newcommand{\UMN}{Minnesota Institute for Astrophysics, University of Minnesota, 116 Church Street SE, Minneapolis, MN 55455, USA}
\newcommand{\Geneva}{Department of Astronomy, University of Geneva, 51, Ch. des Maillettes, CH-1290 Versoix, Switzerland}
\newcommand{\Canarias}{Instituto de Astrofisica de Canarias (IAC), E-38205 La Laguna, Tenerife, Spain}
\newcommand{\Laguna}{Universidad de La Laguna, Dpto. Astrofisica, E-38206 La Laguna, Tenerife, Spain}
\newcommand{\BenGurion}{Physics Department, Ben-Gurion University of the Negev, P.O. Box 653, Beer-Sheva 8410501, Israel}
\newcommand{\CfA}{Harvard-Smithsonian Center for Astrophysics, 60 Garden Street, Cambridge, MA 02138}
\newcommand{\NSF}{NSF Astronomy and Astrophysics Postdoctoral Fellow}
\newcommand{\Miller}{Miller Institute for Basic Research in Science, University of California, Berkeley, CA 94720, USA}
\newcommand{\Kwazulu}{Astrophysics and Cosmology Research Unit, School of Mathematical Sciences, University of KwaZulu-Natal, Durban 4041, South Africa}
\newcommand{\Stromlo}{The Research School of Astronomy and Astrophysics, Mount Stromlo Observatory, Australian National University, Canberra, ACT 2611, Australia}
\newcommand{\Excellence}{National Centre for the Public Awareness of Science, Australian National University, Canberra, ACT 2611, Australia}
\newcommand{\ASTROThreeD}{The ARC Centre of Excellence for All-Sky Astrophysics in 3 Dimension (ASTRO 3D), Australia}
\newcommand{\Toronto}{Department of Astronomy and Astrophysics, University of Toronto, 50 St. George Street, Toronto, ON, M5S 3H4, Canada}
\newcommand{\Cambridge}{Institute of Astronomy and Kavli Institute for Cosmology, Madingley Road, Cambridge, CB3 0HA, UK}
\newcommand{\Portsmouth}{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}
\newcommand{\StatLabCambridge}{Statistical Laboratory, DPMMS, University of Cambridge, Wilberforce Road, Cambridge, CB3 0WB, UK}
\newcommand{\Sorbonne}{Institut d'Astrophysique de Paris, CNRS-Sorbonne Universit\'e, 98 bis boulevard Arago, F-75014 Paris, France}
\newcommand{\ARI}{Astronomisches Rechen-Institut (ARI), Zentrum für Astronomie der Universität Heidelberg (ZAH),  Mönchhofstr. 12-14, 69120 Heidelberg, Germany}
\newcommand{\ISSI}{International Space Science Institute (ISSI), Hallerstrasse 6, 3012 Bern, Switzerland}
\newcommand{\StonyBrook}{Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794, USA}
\newcommand{\Carnegie}{The Observatories of the Carnegie Institution for Science, 813 SantaBarbara Street, Pasadena, CA 91101, USA}

